How Similar Are Elected Politicians and Their Constituents? Quantitative Evidence From Online Social Networks

How similar are politicians to those who vote for them? This is a critical question at the heart of democratic representation and particularly relevant at times when political dissatisfaction and populism are on the rise. To answer this question we compare the online discourse of elected politicians and their constituents. We collect a two and a half years (September 2020 - February 2023) constituency-level dataset for USA and UK that includes: (i) the Twitter timelines (5.6 Million tweets) of elected political representatives (595 UK Members of Parliament and 433 USA Representatives), (ii) the Nextdoor posts (21.8 Million posts) of the constituency (98.4% USA and 91.5% UK constituencies). We find that elected politicians tend to be equally similar to their constituents in terms of content and style regardless of whether a constituency elects a right or left-wing politician. The size of the electoral victory and the level of income of a constituency shows a nuanced picture. The narrower the electoral victory, the more similar the style and the more dissimilar the content is. The lower the income of a constituency, the more similar the content is. In terms of style, poorer constituencies tend to have a more similar sentiment and more dissimilar psychological text traits (i.e. measured with LIWC categories).

==> dump_text.tex <==
To address this, in this paper we ask how similar are politicians to those that they represent?


% \cite{garimella2017long}
% On the other hand, politicians are responsive to the opinions of their constituents and try to discuss topics of interests of their constituents in order to achieve and maintain electoral success in their constituency \cite{sevenans2021public, matsubayashi2013politicians, martelli2023populist}. But, does these similarity in their discourse also exist over social media platforms?


But what does it mean for a politician to be representative of its voters? Are politicians similar in their online discourse as discourse of their constituents? 
% To discuss more similar content? To discuss them in the same manner?  


In this paper we look at these: we wonder how similar politicians are to their voters in terms of the content and style similarity of their online discourse.
\gareth{There seems to be a deluge of informal questions and wonders. Might be better to tone these down. Also, it is repeating what you say later in the explicit RQs.}



% First, we validate whether LIWC category scores between representatives and constituents belong to different distributions.  \textcolor{red}{Finding the independence of the LIWC category scores for Nextdoor and Twitter is essential before looking at the differences in data distribution.
% \gareth{Why?}
% To this purpose, we calculate the mutual information score \cite{peng2005feature} for every LIWC category in the Twitter and Nextdoor datasets.
% The mutual information score shows how dependent or independent two samples are, and it ranges from 0 to 1. Every LIWC category has mutual information scores which vary between 0.08 and 0.13. This suggests that the LIWC category scores for the Nextdoor and Twitter datasets are largely independent of one other.}


\section{LIWC Categories}

% \pb{The size of the electoral victory and the level of income of a constituency does not relate to variations in the differences for  any LIWC category.}
% As in the previous section, we also examine whether the differences in the scores for the LIWC categories vary across constituencies with different levels of income and sizes of political victory.
% To our surprise we do not find strong trends with differences remaining stubbornly stable across the different constituencies (average IDR xxx, variance xxx across victory sizes and average IDR xxx, variance xxx across levels of income \ignacio{this could be a table}).

% Regardless of scores of constituents and elected  politicians for all LIWC categories belonging to different distributions, medians and standard deviation of their differences are less than 2 (with exceptions of root and summary variables LIWC categories). These results imply that although the writing styles of constituents and elected  politicians are different, these differences are not visible through simple absolute differences in scores. 
% \begin{figure}[!h]
% 	\begin{center}
% 		\includegraphics[width=\columnwidth]{figures/liwc_categories_top_5.png}
% 	\end{center}
% 	\caption{Distribution of differences of root and summary variable LIWC categories score of online discourse between constituents and elected  politicians.}
% 	\label{fig:liwc_med_score}
% \end{figure}
% \begin{table*}[!h]
% \begin{adjustbox}{max width=\linewidth}
% \begin{tabular}{|c|cccc|cccc|}
% \hline
%                     & \multicolumn{4}{c|}{\textbf{Winning Majority}}                                                                                                 & \multicolumn{4}{c|}{\textbf{Income}}                                                                                                           \\ \hline
%                     & \multicolumn{2}{c|}{\textbf{USA}}                                                & \multicolumn{2}{c|}{\textbf{UK}}                            & \multicolumn{2}{c|}{\textbf{USA}}                                                & \multicolumn{2}{c|}{\textbf{UK}}                            \\ \hline
%                     & \multicolumn{1}{c|}{\textbf{Left-wing}} & \multicolumn{1}{c|}{\textbf{Right-wing}} & \multicolumn{1}{c|}{\textbf{Left-wing}} & \textbf{Right-wing} & \multicolumn{1}{c|}{\textbf{Left-wing}} & \multicolumn{1}{c|}{\textbf{Right-wing}} & \multicolumn{1}{c|}{\textbf{Left-wing}} & \textbf{Right-wing} \\ \hline
%                     & \multicolumn{1}{c|}{\textbf{IDR}}      & \multicolumn{1}{c|}{\textbf{IDR}}       & \multicolumn{1}{c|}{\textbf{IDR}}      & \textbf{IDR}       & \multicolumn{1}{c|}{\textbf{IDR}}      & \multicolumn{1}{c|}{\textbf{IDR}}       & \multicolumn{1}{c|}{\textbf{IDR}}      & \textbf{IDR}       \\ \hline
% \textbf{Tone}       & \multicolumn{1}{c|}{-6.705}            & \multicolumn{1}{c|}{-2.360}             & \multicolumn{1}{c|}{-8.220}            & 9.410              & \multicolumn{1}{c|}{-2.785}            & \multicolumn{1}{c|}{-6.745}             & \multicolumn{1}{c|}{-1.100}            & -11.295            \\ \hline
% \textbf{Authentic}  & \multicolumn{1}{c|}{-2.000}            & \multicolumn{1}{c|}{-8.015}             & \multicolumn{1}{c|}{2.130}             & 2.970              & \multicolumn{1}{c|}{-2.985}            & \multicolumn{1}{c|}{4.935}              & \multicolumn{1}{c|}{-1.160}            & -4.045             \\ \hline
% \textbf{Analytic}   & \multicolumn{1}{c|}{-3.165}            & \multicolumn{1}{c|}{-0.505}             & \multicolumn{1}{c|}{-0.750}            & 2.14               & \multicolumn{1}{c|}{4.305}             & \multicolumn{1}{c|}{8.040}              & \multicolumn{1}{c|}{2.680}             & -1.310             \\ \hline
% \textbf{Clout}      & \multicolumn{1}{c|}{1.430}             & \multicolumn{1}{c|}{-10.565}            & \multicolumn{1}{c|}{-2.815}            & -2.720             & \multicolumn{1}{c|}{0.915}             & \multicolumn{1}{c|}{3.635}              & \multicolumn{1}{c|}{5.055}             & -0.455             \\ \hline
% \textbf{Linguistic} & \multicolumn{1}{c|}{-0.930}            & \multicolumn{1}{c|}{-0.090}             & \multicolumn{1}{c|}{0.360}             & 2.095              & \multicolumn{1}{c|}{0.520}             & \multicolumn{1}{c|}{2.790}              & \multicolumn{1}{c|}{-0.915}            & -0.985             \\ \hline
% \textbf{i}          & \multicolumn{1}{c|}{-0.520}            & \multicolumn{1}{c|}{-0.705}             & \multicolumn{1}{c|}{-0.330}            & 0.090              & \multicolumn{1}{c|}{0.155}             & \multicolumn{1}{c|}{1.015}              & \multicolumn{1}{c|}{0.045}             & -0.295             \\ \hline
% \textbf{we}         & \multicolumn{1}{c|}{0.265}             & \multicolumn{1}{c|}{-0.150}             & \multicolumn{1}{c|}{0.010}             & -0.085             & \multicolumn{1}{c|}{0.205}             & \multicolumn{1}{c|}{-0.590}             & \multicolumn{1}{c|}{0.160}             & 0.095              \\ \hline
% \textbf{emo\_pos}   & \multicolumn{1}{c|}{-0.001}            & \multicolumn{1}{c|}{-0.030}             & \multicolumn{1}{c|}{-0.155}            & -0.145             & \multicolumn{1}{c|}{0.020}             & \multicolumn{1}{c|}{0.065}              & \multicolumn{1}{c|}{-0.085}            & 0.001              \\ \hline
% \textbf{emo\_neg}   & \multicolumn{1}{c|}{-0.025}            & \multicolumn{1}{c|}{-0.165}             & \multicolumn{1}{c|}{0.110}             & 0.465              & \multicolumn{1}{c|}{0.135}             & \multicolumn{1}{c|}{-0.075}             & \multicolumn{1}{c|}{-0.030}            & 0.050              \\ \hline
% \textbf{emo\_anx}   & \multicolumn{1}{c|}{0.001}             & \multicolumn{1}{c|}{0.001}              & \multicolumn{1}{c|}{0.001}             & 0.005              & \multicolumn{1}{c|}{0.001}             & \multicolumn{1}{c|}{0.010}              & \multicolumn{1}{c|}{0.001}             & 0.020              \\ \hline
% \textbf{feeling}    & \multicolumn{1}{c|}{-0.005}            & \multicolumn{1}{c|}{0.001}              & \multicolumn{1}{c|}{-0.005}            & 0.010              & \multicolumn{1}{c|}{0.015}             & \multicolumn{1}{c|}{0.020}              & \multicolumn{1}{c|}{0.050}             & 0.045              \\ \hline
% \textbf{tentat}     & \multicolumn{1}{c|}{0.115}             & \multicolumn{1}{c|}{0.190}              & \multicolumn{1}{c|}{-0.150}            & 0.065              & \multicolumn{1}{c|}{0.115}             & \multicolumn{1}{c|}{-0.030}             & \multicolumn{1}{c|}{0.115}             & -0.225             \\ \hline
% \textbf{certitude}  & \multicolumn{1}{c|}{0.005}             & \multicolumn{1}{c|}{0.055}              & \multicolumn{1}{c|}{-0.020}            & -0.060             & \multicolumn{1}{c|}{0.025}             & \multicolumn{1}{c|}{0.055}              & \multicolumn{1}{c|}{0.040}             & 0.045              \\ \hline
% \textbf{achieve}    & \multicolumn{1}{c|}{0.285}             & \multicolumn{1}{c|}{0.145}              & \multicolumn{1}{c|}{0.065}             & -0.190             & \multicolumn{1}{c|}{0.200}             & \multicolumn{1}{c|}{-0.395}             & \multicolumn{1}{c|}{0.100}             & 0.235              \\ \hline
% \textbf{relig}      & \multicolumn{1}{c|}{0.020}             & \multicolumn{1}{c|}{-0.065}             & \multicolumn{1}{c|}{0.025}             & -0.010             & \multicolumn{1}{c|}{-0.015}            & \multicolumn{1}{c|}{-0.025}             & \multicolumn{1}{c|}{0.035}             & 0.050              \\ \hline
% \textbf{death}      & \multicolumn{1}{c|}{-0.030}            & \multicolumn{1}{c|}{-0.035}             & \multicolumn{1}{c|}{-0.045}            & 0.010              & \multicolumn{1}{c|}{-0.040}            & \multicolumn{1}{c|}{-0.080}             & \multicolumn{1}{c|}{0.015}             & -0.040             \\ \hline
% \end{tabular}
% \end{adjustbox}
% \label{tab:liwc_idr}
% \caption{Inter-decile range for LIWC categories}
% \end{table*}


% \begin{figure}[!h]
%     \begin{center}
%         \includegraphics[width=\columnwidth]{figures/liwc_categories_top_5.png}
%     \end{center}
%     \caption{Distribution of differences of root and summary variable LIWC categories score of online discourse between constituents and elected politicians.}
%     \label{fig:liwc_med_score}
% \end{figure}






% \begin{table*}[!h]
% \begin{adjustbox}{max width=\linewidth}
% \begin{tabular}{|c|cccccccc|cccccccc|}
% \hline
% \multirow{4}{*}{\textbf{}} & \multicolumn{8}{c|}{\textbf{Income}}                                                                                                                                                                                                                                         & \multicolumn{8}{c|}{\textbf{Winning Majority}}                                                                                                                                                                                                                               \\ \cline{2-17} 
%                            & \multicolumn{4}{c|}{\textbf{USA}}                                                                                                               & \multicolumn{4}{c|}{\textbf{UK}}                                                                                           & \multicolumn{4}{c|}{\textbf{USA}}                                                                                                               & \multicolumn{4}{c|}{\textbf{UK}}                                                                                           \\ \cline{2-17} 
%                            & \multicolumn{2}{c|}{\textbf{Left-wing}}                                 & \multicolumn{2}{c|}{\textbf{Right-wing}}                                & \multicolumn{2}{c|}{\textbf{Left-wing}}                                 & \multicolumn{2}{c|}{\textbf{Right-wing}}           & \multicolumn{2}{c|}{\textbf{Left-wing}}                                 & \multicolumn{2}{c|}{\textbf{Right-wing}}                                & \multicolumn{2}{c|}{\textbf{Left-wing}}                                 & \multicolumn{2}{c|}{\textbf{Right-wing}}           \\ \cline{2-17} 
%                            & \multicolumn{1}{c|}{\textbf{Slope}} & \multicolumn{1}{c|}{\textbf{r\textsuperscript{2}}} & \multicolumn{1}{c|}{\textbf{Slope}} & \multicolumn{1}{c|}{\textbf{r\textsuperscript{2}}} & \multicolumn{1}{c|}{\textbf{Slope}} & \multicolumn{1}{c|}{\textbf{r\textsuperscript{2}}} & \multicolumn{1}{c|}{\textbf{Slope}} & \textbf{r\textsuperscript{2}} & \multicolumn{1}{c|}{\textbf{Slope}} & \multicolumn{1}{c|}{\textbf{r\textsuperscript{2}}} & \multicolumn{1}{c|}{\textbf{Slope}} & \multicolumn{1}{c|}{\textbf{r\textsuperscript{2}}} & \multicolumn{1}{c|}{\textbf{Slope}} & \multicolumn{1}{c|}{\textbf{r\textsuperscript{2}}} & \multicolumn{1}{c|}{\textbf{Slope}} & \textbf{r\textsuperscript{2}} \\ \hline
% \textbf{Tone}              & \multicolumn{1}{c|}{-6.483}         & \multicolumn{1}{c|}{0.664}       & \multicolumn{1}{c|}{-6.961}         & \multicolumn{1}{c|}{0.784}       & \multicolumn{1}{c|}{7.227}          & \multicolumn{1}{c|}{0.802}       & \multicolumn{1}{c|}{6.265}          & 0.723       & \multicolumn{1}{c|}{-6.214}         & \multicolumn{1}{c|}{0.629}       & \multicolumn{1}{c|}{-7.063}         & \multicolumn{1}{c|}{0.788}       & \multicolumn{1}{c|}{-7.432}         & \multicolumn{1}{c|}{0.788}       & \multicolumn{1}{c|}{6.007}          & 0.727       \\ \hline
% \textbf{Authentic}         & \multicolumn{1}{c|}{-4.700}         & \multicolumn{1}{c|}{0.734}       & \multicolumn{1}{c|}{5.044}          & \multicolumn{1}{c|}{0.841}       & \multicolumn{1}{c|}{3.695}          & \multicolumn{1}{c|}{0.804}       & \multicolumn{1}{c|}{-4.121}         & 0.750       & \multicolumn{1}{c|}{-4.595}         & \multicolumn{1}{c|}{0.722}       & \multicolumn{1}{c|}{-4.987}         & \multicolumn{1}{c|}{0.802}       & \multicolumn{1}{c|}{-3.803}         & \multicolumn{1}{c|}{0.791}       & \multicolumn{1}{c|}{-3.947}         & 0.751       \\ \hline
% \textbf{Analytic}          & \multicolumn{1}{c|}{4.376}          & \multicolumn{1}{c|}{0.760}       & \multicolumn{1}{c|}{4.766}          & \multicolumn{1}{c|}{0.860}       & \multicolumn{1}{c|}{3.006}          & \multicolumn{1}{c|}{0.790}       & \multicolumn{1}{c|}{-3.749}         & 0.742       & \multicolumn{1}{c|}{4.254}          & \multicolumn{1}{c|}{0.739}       & \multicolumn{1}{c|}{-4.640}         & \multicolumn{1}{c|}{0.795}       & \multicolumn{1}{c|}{-3.055}         & \multicolumn{1}{c|}{0.758}       & \multicolumn{1}{c|}{3.625}          & 0.758       \\ \hline
% \textbf{Clout}             & \multicolumn{1}{c|}{2.072}          & \multicolumn{1}{c|}{0.646}       & \multicolumn{1}{c|}{-1.404}         & \multicolumn{1}{c|}{0.524}       & \multicolumn{1}{c|}{-1.179}         & \multicolumn{1}{c|}{0.543}       & \multicolumn{1}{c|}{-1.824}         & 0.569       & \multicolumn{1}{c|}{2.101}          & \multicolumn{1}{c|}{0.684}       & \multicolumn{1}{c|}{-1.399}         & \multicolumn{1}{c|}{0.508}       & \multicolumn{1}{c|}{-1.221}         & \multicolumn{1}{c|}{0.540}       & \multicolumn{1}{c|}{1.798}          & 0.604       \\ \hline
% \textbf{Linguistic}        & \multicolumn{1}{c|}{1.629}          & \multicolumn{1}{c|}{0.750}       & \multicolumn{1}{c|}{1.836}          & \multicolumn{1}{c|}{0.838}       & \multicolumn{1}{c|}{1.074}          & \multicolumn{1}{c|}{0.759}       & \multicolumn{1}{c|}{-1.416}         & 0.720       & \multicolumn{1}{c|}{-1.559}         & \multicolumn{1}{c|}{0.707}       & \multicolumn{1}{c|}{-1.820}         & \multicolumn{1}{c|}{0.804}       & \multicolumn{1}{c|}{1.105}          & \multicolumn{1}{c|}{0.747}       & \multicolumn{1}{c|}{-1.359}         & 0.724       \\ \hline
% \textbf{i}                 & \multicolumn{1}{c|}{0.313}          & \multicolumn{1}{c|}{0.707}       & \multicolumn{1}{c|}{0.341}          & \multicolumn{1}{c|}{0.809}       & \multicolumn{1}{c|}{-0.270}         & \multicolumn{1}{c|}{0.761}       & \multicolumn{1}{c|}{-0.282}         & 0.733       & \multicolumn{1}{c|}{-0.293}         & \multicolumn{1}{c|}{0.636}       & \multicolumn{1}{c|}{-0.325}         & \multicolumn{1}{c|}{0.719}       & \multicolumn{1}{c|}{-0.273}         & \multicolumn{1}{c|}{0.724}       & \multicolumn{1}{c|}{0.276}          & 0.766       \\ \hline
% \textbf{we}                & \multicolumn{1}{c|}{0.116}          & \multicolumn{1}{c|}{0.568}       & \multicolumn{1}{c|}{-0.064}         & \multicolumn{1}{c|}{0.451}       & \multicolumn{1}{c|}{-0.049}         & \multicolumn{1}{c|}{0.527}       & \multicolumn{1}{c|}{-0.075}         & 0.505       & \multicolumn{1}{c|}{0.121}          & \multicolumn{1}{c|}{0.628}       & \multicolumn{1}{c|}{-0.064}         & \multicolumn{1}{c|}{0.450}       & \multicolumn{1}{c|}{-0.050}         & \multicolumn{1}{c|}{0.521}       & \multicolumn{1}{c|}{0.073}          & 0.531       \\ \hline
% \textbf{emo\_pos}          & \multicolumn{1}{c|}{-0.043}         & \multicolumn{1}{c|}{0.530}       & \multicolumn{1}{c|}{0.058}          & \multicolumn{1}{c|}{0.380}       & \multicolumn{1}{c|}{0.044}          & \multicolumn{1}{c|}{0.620}       & \multicolumn{1}{c|}{-0.039}         & 0.492       & \multicolumn{1}{c|}{-0.042}         & \multicolumn{1}{c|}{0.520}       & \multicolumn{1}{c|}{-0.054}         & \multicolumn{1}{c|}{0.320}       & \multicolumn{1}{c|}{-0.044}         & \multicolumn{1}{c|}{0.570}       & \multicolumn{1}{c|}{-0.037}         & 0.485       \\ \hline
% \textbf{emo\_neg}          & \multicolumn{1}{c|}{-0.264}         & \multicolumn{1}{c|}{0.726}       & \multicolumn{1}{c|}{-0.274}         & \multicolumn{1}{c|}{0.828}       & \multicolumn{1}{c|}{0.237}          & \multicolumn{1}{c|}{0.819}       & \multicolumn{1}{c|}{-0.298}         & 0.774       & \multicolumn{1}{c|}{0.265}          & \multicolumn{1}{c|}{0.752}       & \multicolumn{1}{c|}{0.277}          & \multicolumn{1}{c|}{0.830}       & \multicolumn{1}{c|}{0.248}          & \multicolumn{1}{c|}{0.831}       & \multicolumn{1}{c|}{-0.282}         & 0.756       \\ \hline
% \textbf{emo\_anx}          & \multicolumn{1}{c|}{0.005}          & \multicolumn{1}{c|}{0.552}       & \multicolumn{1}{c|}{0.005}          & \multicolumn{1}{c|}{0.606}       & \multicolumn{1}{c|}{0.003}          & \multicolumn{1}{c|}{0.444}       & \multicolumn{1}{c|}{0.007}          & 0.565       & \multicolumn{1}{c|}{0.005}          & \multicolumn{1}{c|}{0.527}       & \multicolumn{1}{c|}{-0.005}         & \multicolumn{1}{c|}{0.552}       & \multicolumn{1}{c|}{0.003}          & \multicolumn{1}{c|}{0.415}       & \multicolumn{1}{c|}{0.006}          & 0.591       \\ \hline
% \textbf{feeling}           & \multicolumn{1}{c|}{0.023}          & \multicolumn{1}{c|}{0.697}       & \multicolumn{1}{c|}{-0.022}         & \multicolumn{1}{c|}{0.750}       & \multicolumn{1}{c|}{0.029}          & \multicolumn{1}{c|}{0.765}       & \multicolumn{1}{c|}{0.037}          & 0.667       & \multicolumn{1}{c|}{-0.022}         & \multicolumn{1}{c|}{0.654}       & \multicolumn{1}{c|}{0.023}          & \multicolumn{1}{c|}{0.777}       & \multicolumn{1}{c|}{0.029}          & \multicolumn{1}{c|}{0.696}       & \multicolumn{1}{c|}{0.035}          & 0.654       \\ \hline
% \textbf{tentat}            & \multicolumn{1}{c|}{0.386}          & \multicolumn{1}{c|}{0.750}       & \multicolumn{1}{c|}{-0.392}         & \multicolumn{1}{c|}{0.833}       & \multicolumn{1}{c|}{0.319}          & \multicolumn{1}{c|}{0.828}       & \multicolumn{1}{c|}{-0.397}         & 0.777       & \multicolumn{1}{c|}{0.386}          & \multicolumn{1}{c|}{0.772}       & \multicolumn{1}{c|}{0.398}          & \multicolumn{1}{c|}{0.840}       & \multicolumn{1}{c|}{-0.329}         & \multicolumn{1}{c|}{0.819}       & \multicolumn{1}{c|}{0.381}          & 0.780       \\ \hline
% \textbf{certitude}         & \multicolumn{1}{c|}{0.018}          & \multicolumn{1}{c|}{0.482}       & \multicolumn{1}{c|}{0.014}          & \multicolumn{1}{c|}{0.604}       & \multicolumn{1}{c|}{0.015}          & \multicolumn{1}{c|}{0.568}       & \multicolumn{1}{c|}{0.018}          & 0.566       & \multicolumn{1}{c|}{0.018}          & \multicolumn{1}{c|}{0.522}       & \multicolumn{1}{c|}{-0.014}         & \multicolumn{1}{c|}{0.565}       & \multicolumn{1}{c|}{0.015}          & \multicolumn{1}{c|}{0.561}       & \multicolumn{1}{c|}{-0.016}         & 0.478       \\ \hline
% \textbf{achieve}           & \multicolumn{1}{c|}{0.138}          & \multicolumn{1}{c|}{0.660}       & \multicolumn{1}{c|}{0.113}          & \multicolumn{1}{c|}{0.721}       & \multicolumn{1}{c|}{0.044}          & \multicolumn{1}{c|}{0.648}       & \multicolumn{1}{c|}{-0.085}         & 0.608       & \multicolumn{1}{c|}{0.145}          & \multicolumn{1}{c|}{0.752}       & \multicolumn{1}{c|}{0.116}          & \multicolumn{1}{c|}{0.737}       & \multicolumn{1}{c|}{0.046}          & \multicolumn{1}{c|}{0.654}       & \multicolumn{1}{c|}{-0.079}         & 0.563       \\ \hline
% \textbf{relig}             & \multicolumn{1}{c|}{0.015}          & \multicolumn{1}{c|}{0.425}       & \multicolumn{1}{c|}{0.013}          & \multicolumn{1}{c|}{0.357}       & \multicolumn{1}{c|}{-0.012}         & \multicolumn{1}{c|}{0.138}       & \multicolumn{1}{c|}{0.016}          & 0.218       & \multicolumn{1}{c|}{-0.012}         & \multicolumn{1}{c|}{0.273}       & \multicolumn{1}{c|}{-0.013}         & \multicolumn{1}{c|}{0.325}       & \multicolumn{1}{c|}{-0.011}         & \multicolumn{1}{c|}{0.115}       & \multicolumn{1}{c|}{-0.013}         & 0.159       \\ \hline
% \textbf{death}             & \multicolumn{1}{c|}{0.018}          & \multicolumn{1}{c|}{0.538}       & \multicolumn{1}{c|}{-0.013}         & \multicolumn{1}{c|}{0.534}       & \multicolumn{1}{c|}{0.015}          & \multicolumn{1}{c|}{0.539}       & \multicolumn{1}{c|}{-0.013}         & 0.364       & \multicolumn{1}{c|}{-0.016}         & \multicolumn{1}{c|}{0.417}       & \multicolumn{1}{c|}{0.014}          & \multicolumn{1}{c|}{0.588}       & \multicolumn{1}{c|}{-0.015}         & \multicolumn{1}{c|}{0.472}       & \multicolumn{1}{c|}{-0.012}         & 0.350       \\ \hline
% \end{tabular}
% \end{adjustbox}
% \label{tab:liwc_reg}
% \caption{Regression parameters for LIWC categories}
% \end{table*}






% Sylwester et al. verified that several LIWC categories are good identifiers of  left-wing and right-wing political orientation \cite{sylwester2015twitter}. 
% % These LIWC categories include ``1st person singular pronoun (i)'', ``1st person plural noun (we)'', ``swear words (swear)'', ``positive sentiment (emo$\_$pos), ``negative sentiment (emo$\_$neg)'',``Anxiety (emo$\_$aux)'', ``Feeling (feel)'', ``tentative (tentat)'', ``centainty (certitude)'', ``achievment (achieve)'', religion (relig)'', and ``death (death)''. 
% We also analyze these categories and observe that median and standard deviation for these categories are also small ($<2$). 
% These categories seemingly identify equally well the political colour of a constituency through its elected  politicians or constituents.

% We also observe that there are some root and summary variables LIWC categories where difference in constituents and representaives scores is higher than rest. Figure \ref{fig:liwc_med_score} represents distribution of root and summary variables LIWC categories scores which are prominently higher than the rest of the LIWC categories. We observe that linguistic-based \ie~ \emph{Tone, Analytic, Clout, Authentic, and Linguistic} LIWC categories can more prominently represent difference in constituents' and elected  politicians' writing styles.


==> findings.tex <==
Topic similarities

1. {first pb}  We find that elected politicians and constituents discuss similar topics in their constituency regardless of whether a constituency is right or left-wing, although in a slightly different order and size. The close-to-zero variance indicates that this is the case for most constituencies.
2. {Second pb} Elected politicians and their constituents discuss similar topics regardless of how contested a constituency is or the level of income. This trend is similar in both the USA and UK

Semantic similarity

1. {first pb} Right and left-wing elected politicians discuss similar issues to their constituents
2. {Second pb} Elected politicians in less disputed constituencies have a more similar discourse to their constituents. This is particularly in the UK and right-wing USA constituencies. 
3. {Third pb} Elected politicians of poorer constituencies have more similar discourse to their constituents. 
4. {Forth pb} Elected politicians have low discourse similarity with constituents that they do not represent. he level of similarity between constituents and politicians of different political signs is lower than when we conducted within constituency comparisons. 


Style-related similarities
Psychological similarities
1. {First pb} Elected politicians have a similar discourse style as of their constituents regardless of political ideology. Differences of discourse style between right-wing and left-wing constituencies are small even when significant. 
2. {Second pb} Elected politicians of more disputed constituencies have more similar discourse style to constituents. Depending on size of the winning majority, we observe that the IDR values of our analyzed LIWC scores are negative in left-wing and right-wing constituencies in the USA and left-wing constituencies in UK, but positive in right-wing constituencies in the UK.
3. {Third pb} Elected politicians in richer constituencies tend to have more similar style to their constituents. We also observe that the similarity in style decreases in lower-income constituencies except for right-wing constituencies in the UK.

Sentiment similarity
1. {first pb} The narrower the majority, the more similar the sentiment between elected politicians and their constituents. This is true for both countries and across the political spectrum.
2. {second pb} Elected politicians from poorer constituencies have more similar sentiment to their constituents.


%%%%%%%%%%%%
Summarised

We find that elected politicians tend to be equally similar to their constituents in terms of content and style regardless of whether a constituency elects a right or left-wing politician. 
The size of the electoral victory and the level of income of a constituency  shows a nuanced picture.
The narrower the electoral victory,
the more similar the style and the more dissimilar the content is. 
The lower the income of a constituency,
the more similar content is. 
In terms of style, 
poorer constituencies tend to have a more similar sentiment and
more dissimilar psychological text traits (\ie measured with LIWC categories).

==> icwsm24-winter-reviews.tex <==
https://docs.google.com/document/d/1W9GuU123axakqb_q7AWx-6EY2RHOBbZAXn5nxkuFlUo/edit?pli=1

===================Reviews for your paper follow===================

----------------------------------------------------------------

SPC/Associate Editor review (reviewer 4)

  Second Round Comments for Authors

    (blank)

  Ethical concerns summary

    None spotted

  Meta-Review and Roadmap

    This paper performs a large-scale comparative analysis of content posted on
    Nextdoor and Twitter to study similarities and differences in themes and styles
    between politicians and their constituents in the UK and the US.


    Reviewers value the following aspects of the paper:
    - Use of NextDoor data (due to a lack of focus on this platform in previous
    studies) and the geographical mapping between neighbourhoods and constituencies
    - Overall well written

    However, the reviewers also see weaknesses and shortcomings that leave room for
    improvement:
    - Motivation could be clearer
    - No detailed discussion and/or validation of the "representativeness claim"
    - Methodological reservations concerning the sentiment and cosine similarity
    calculations


    The reviewers invite the authors to revise and resubmit their work and consider
    the following points:
    The authors should revise the comparison of language use by focusing on two
    aspects: How does noise, in other words, the creation of the word vectors, play a
    role in the cosine similarity calculations? They could possibly consider related
    work that has focused on this aspect.
    - How does topic similarity affect the similarity in language use between left-
    wing citizens and right-wing politicians and vice-versa.
    Overall, the reviews highlight the need for more clarity in certain parts of the
    paper.
    - Secondly, the 'representativeness claim' warrants further analysis that either
    documents this representativeness or there is at least a need for further
    discussion and reflections of the possible limitations that are associated with
    it.

----------------------------------------------------------------

reviewer/PC member review (reviewer 1)

  Second Round Comments for Authors

    (blank)

  Overall evaluation

    -2 = Reject: For instance, a paper with limited social impact, insufficient
    evaluation, poor reproducibility, technical issues, or issues with unaddressed
    ethical considerations.

  Reviewer's Confidence

    4 = Quite confident. I tried to check the important points carefully. It is
    unlikely, though conceivable, that I missed some aspects that could otherwise have
    impacted my evaluation.

  Reviewer's methodological expertise

    5 = Very Knowledgeable: This paper significantly overlaps with my current work and
    I am very knowledgeable about most of the topics covered by the paper.

  Paper summary

    This paper compares posts on Nextdoor to politicians’ posts in the same
    constituencies on Twitter. It assesses online post content alignment between
    constituents and their political representatives. The authors make a series of
    claims about similarities by left vs right wing (scored by representative party
    affiliation), election competitiveness, and constituency income.

  Reasons to accept

    The main strength of this paper is its use of Nextdoor data in both the US and UK.
    This is probably a politically important website, especially for local issues, and
    it is far less studied than Twitter.

  Reasons to reject

    Many of the interpretations are not clearly substantiated and some are likely to
    be false.

    The authors are trying to compare language use across Twitter (for politicians)
    and Nextdoor (for constituents). They claim that Nextdoor is representative of
    constituents but only based on correlations between number of users/posts and
    population. It's unlikely that language use will match across platforms,
    especially if the user bases are different, and so I'm not sure what comparisons
    across these platforms will mean.

    The cosine similarity calculations on averages are a mix of noise (depending on
    the number of averaged vectors, which is determined by population size) and actual
    effects. I do not know how much that will matter. Repeated pairwise comparisons,
    with benchmarks for within constituency versus not, would have been more
    informative. I have provided the authors a citation on that.

    The authors have not stated how the error bars were calculated or if they
    represent for example 1 standard error or 2.  They seem to be automated output
    from some sort of smoother. But I'm not sure how much this matters given the
    broader issues with trying to compare across platforms and different users bases.

  Comments for authors

    This paper compares posts on Nextdoor to politicians’ posts in the same
    constituencies on Twitter. Its stated goal is to assess online post content
    alignment between constituents and their political representatives. The authors
    make a series of claims about similarities by left vs right wing (scored by
    representative party affiliation), election competitiveness, and constituency
    income.

    The main strength of this paper is its use of Nextdoor data in both the US and the
    UK. This is probably a politically important website, especially for local issues,
    and it is far less studied than Twitter. Simply because of that I am favorably
    inclined toward most research on Nextdoor. I think the most impressive part of
    this effort is the data collection and the mapping of neighborhoods to
    constituencies. However, I think this paper uses data from a previous work that
    had already done that.

    The paper also constructs several different measures for scoring similarity and
    that can be used to assess various aspects of language use.

    The main weaknesses of this paper are related to the analyses and interpretations.
    Many of the interpretations are not clearly substantiated and some are likely to
    be false.

    1. The cosine similarity calculations on averaged vectors are a mix of noise
    (depending on the number of averaged vectors, which is strongly affected by
    population size) and actual effects. I do not know how much that will matter.
    Repeated pairwise comparisons, with benchmarks for within constituency versus not,
    would have been more informative. Noise drives cosine similarity toward 0. This
    effect might not be very large but none of the stated differences with variables
    are large relative to the error bars (1 or 2 standard errors? How were they
    calculated? Are these just from a smoother?). As a reference for a method that
    accounts for these sorts of effects, see “Lexical Ambiguity in Political Rhetoric”
    by Kraft and Klemmensen.

    2. The authors claim that Nextdoor is representative of constituents but only
    assess correlation between population sizes. This seems to repeat and expand
    similarly unsubstantiated claims in the cited Iqbal et al. 2023. Population size
    is pretty much always extremely strongly correlated in these sorts of analyses,
    and it is a very poor indicator of representativeness more broadly. Also, even if
    users were representative,  who posts the most might not be.

    3. The authors are trying to compare language use across Twitter (for politicians)
    and Nextdoor (for constituents). It's unlikely that language use will match across
    platforms, especially if the user bases are very different (and usually social
    media platforms do have very different active user bases), and so I'm not sure
    what comparisons across these platforms will mean. A study of both politicians and
    constituents on Nextdoor would have provided much more interpretable findings.
    This issue should have been directly discussed and addressed in some way.

    4. The LIWC analyses are difficult to assess since it sounds like the authors have
    reported only differences that were above some sort of threshold? And these
    categories also seem to be the more proprietary (also less fully explained and, in
    my experience anyway, very different distributions) summary ones in LIWC?

    5. Many statistical tests will be invalid with repeated observations from the same
    people, unless there’s something done to account for non-independence. I think
    there is only one formal statistical test in this paper (whether constituents on
    Nextdoor and politicians on Twitter use different language) and I do not see an
    indication that that test accounts for non-independence (I’m pretty sure the KS
    test relies on IID data).

    The paper could be more focused in its motivation. For example, the authors ask
    “What does it mean for a politician to be representative of its voters?”. The most
    common answer to this question is how well a political official represents the
    interests of their constituents. This does not have to be reflected in language
    use. There are studies that assess more specific questions related to this and
    that are more precise in assessing why similarities in language use matters. See,
    for example, “Who Leads? Who Follows? Measuring Issue Attention and Agenda Setting
    by Legislators and the Mass Public Using Social Media Data”. (this didn’t need to
    be cited necessarily since it doesn't quite fit here but I think it might be
    helpful in more clearly motivating these sorts of analyses)

    One last thing – the competitiveness analysis seems interesting but should this
    vary in meaning across the US and UK? I would think the different party sizes and
    dynamics should matter.

  Originality of work

    This broad topic has been studied many times.

    But Nextdoor is extremely important, understudied, and potentially unique and so I
    don't think it matters whether the topic broadly has been studied with other data.

  Potential impact of results

    Unclear due to methodological concerns.

  Quality of execution

    See comments to author

  Quality of presentation

    There are many results that could be presented more cohesively.

  Adequacy of citations

    They didn't have to cite more papers but I've still recommended some that they
    might use to improve the statistical analyses and to better motivate what exactly
    they are trying to study.

  Ethical concerns (if any)

    (blank)

----------------------------------------------------------------

reviewer/PC member review (reviewer 2)

  Second Round Comments for Authors

    (blank)

  Overall evaluation

    -1 = Weak Reject: Technically solid paper where reasons to reject, e.g., fair/poor
    problem significance and social impact, outweigh reasons to accept, e.g. good
    quality.

  Reviewer's Confidence

    4 = Quite confident. I tried to check the important points carefully. It is
    unlikely, though conceivable, that I missed some aspects that could otherwise have
    impacted my evaluation.

  Reviewer's methodological expertise

    5 = Very Knowledgeable: This paper significantly overlaps with my current work and
    I am very knowledgeable about most of the topics covered by the paper.

  Paper summary

    This paper seeks to examine how similar politicians (in the US and UK) are to
    their constituents by analyzing the content and style similarity of their online
    discourse using about 2 and a half years worth of Twitter (X) and Nextdoor data.
    Moreover, the authors also take into account constituency income levels and the
    impact of contested elections.

  Reasons to accept

    The use of Nextdoor data as a proxy for constituencies is very clever, though
    might have some imperfections. The additional analyses for income level and
    contested elections makes the paper even more interesting.

  Reasons to reject

    LIWC, as a dictionary based method, may not encompass all of the necessary terms
    that might help distinguish similarities and differences of interest here. VADER,
    too, is highly dictionary dependent – so while it’s good for social media data, it
    would have been interesting to include other sentiment analysis scores derived by
    other means.

  Comments for authors

    (blank)

  Originality of work

    Somewhat original and with higher chances of novelty in the future.

  Potential impact of results

    This paper is setting up for some really interesting future research, especially
    in cases where researchers are interested in constituencies but aren’t sure how to
    derive that information. Again, I really enjoyed the use of Next door data as a
    proxy – that method has room for improvement but is really smart. I can’t say the
    results are particularly impactful, but as the researchers dig in this has a lot
    of potential.

  Quality of execution

    Overall, well executed.

  Quality of presentation

    Flow/organization of paper seemed a bit disjointed with the related works at the
    end. Minor writing errors (e.g. section header "Style-related similarities
    similarities"). Not enough to take away from the overall argument and outline of
    the work.

  Adequacy of citations

    More ICWSM might have been useful, but the chosen citations cover the information
    provided in text.

  Ethical concerns (if any)

    (blank)

----------------------------------------------------------------

reviewer/PC member review (reviewer 3)

  Second Round Comments for Authors

    (blank)

  Overall evaluation

    0 = Borderline: No real problems with the paper quality and paper presentation,
    but limited impact, limited problem significance, or limited technical novelty

  Reviewer's Confidence

    4 = Quite confident. I tried to check the important points carefully. It is
    unlikely, though conceivable, that I missed some aspects that could otherwise have
    impacted my evaluation.

  Reviewer's methodological expertise

    4 = Knowledgeable: This paper has some overlap with my current work. My recent
    work was focused on closely related topics and I am knowledgeable about most of
    the topics covered by the paper.

  Paper summary

    This work explores the alignment between the online discourse of elected
    politicians and their constituents in the UK and USA. By analyzing 5.6 million
    tweets from politicians and 21.8 million Nextdoor posts from constituents, it
    finds that politicians are broadly representative in terms of content and style,
    regardless of political affiliation.

  Reasons to accept

    This work provides significant contribution to understanding the alignment between
    the online discourse of elected politicians and their constituents, offering
    valuable insights into political representativeness on social media. It provides a
    nuanced view of how content and style of communication vary across different
    political spectrums and constituency characteristics.  Their findings provide
    valueable insight to Political Science.

  Reasons to reject

    There are some methodology details that are unclear and should be clarified or
    modified. However, I do think that these issues can be addressed in the next step
    of revision and do not need to be a reason to reject.

  Comments for authors

    Dear Authors,

    Thank you for sharing your work, it is a very interesting paper.

    However, there are a few points that were not quite clear to me or seemed somewhat
    weaker compared to the rest of the paper. I have listed these points below:

     - It would be beneficial to explain how preprocessing was performed in text
    embeddings in the “Feature Engineering” subsection with 1-2 sentences.

     - The y-axis name on Figure 2 is missing. What does the y-axis represent? Is it
    percentage? It would be good to indicate this.

     - Also, regarding Figure 2, my understanding is that left-wing and right-wing on
    Twitter are discussing the same topics, and left-wing and right-wing on Nextdoor
    are discussing the same topics, rather than left-wing on Twitter and Nextdoor
    discussing the same topics, etc. It would be clearer to present this part in
    another way to directly support your claim.

     - The content in Table 3 could be presented as a figure to increase clarity.

     - Figure 3 and 4 show the distribution of cosine similarity of mean-pooled
    textual embeddings between constituents and representatives. However, given that
    the topics discussed by left-wing and right-wing are so similar, it’s hard to
    determine whether there are consistencies within left-wing and right-wing groups
    respectively. It would be beneficial to show the cosine similarity between left-
    wing constituents and right-wing representatives, as well as between right-wing
    constituents and left-wing representatives, to increase the robustness of your
    claim.

     - The authors should consider modifying the figure layout throughout the paper.
    Figures should be positioned at the top or bottom of the page on which they are
    mentioned.

     - Minor typos/formatting issues:
    There is an extra “left-wing” at the end of line 4 in the third paragraph on the
    right side of page 2.
    There are a few citations (e.g., in the "Nextdoor Data" subsection, “We classify
    them into right and left-wing as in (Jolly et al. 2022). Three small parties are
    not included in (Jolly et al. 2022): …”) that should not be within parentheses.

  Originality of work

    (blank)

  Potential impact of results

    (blank)

  Quality of execution

    (blank)

  Quality of presentation

    (blank)

  Adequacy of citations

    (blank)

  Ethical concerns (if any)

    (blank)

----------------------------------------------------------------




==


==> intro-old.tex <==
\section{Introduction}
During elections, politicians tend to make their political campaign closest to political issues of their voters \cite{cruz2024making, schipper2018political}. They do not just focus on what they are saying is relevant to the political needs of their voters, but, also how they are saying which can effectively convey their message to their constituents~\cite{parmelee2023personalization, bischof2018simple}. After elections, voters' also expect from elected politicians to remain representative of their political issues after election~\cite{giger2021policy}. 

But, recent survey data show voters do not think their elected politicians are representative of their political issues. Many people worldwide see room for improvement in how elected politicians represent them~\cite{views-political-representation}.
Would the situation improve if politicians were more similar to those that they represent? Recent survey data seems to point in that direction. 66\% of USA adults say it is extremely or very important that their political representatives share their views on political issues~\cite{representative-views}. 

% Another survey data shows that 77\% out of 31K interviewed people from 24 different countries prefer representative democracy and show different views on who can represent them better. People from left political ideology shown inclination that their politicians will be more representative if they are labor union members, young adults, people from poor backgrounds and women. Whereas people from right ideology shown preference for electing religious and business persons as their representative~\cite{representative-democracy}. \ignacio{is this statement correct? are there pointers we can throw here?} \waleed{similar in what sense? financially, education wise?}
%

A widespread belief is out there that politicians are out of touch and disconnected from the lives of ordinary citizens in current state of representative democracy. Many have argued that politicians are becoming less representative and this is indeed a problem. \citeauthor{jones2020chavs} \cite{jones2020chavs} argues that left-wing politicians are increasingly less representative of those with lower incomes that they are supposed to represent. Piketty~\cite{piketty2018brahmin} has also shown how support for left-wing parties has indeed shifted across western countries. With growing political polarization \cite{garimella2017long} and the rise of populism \cite{martelli2023populist, populists-pew}, it is crucial to understand the scale of how much politicians represent and focus on political issues their voters favor.

To understand how representative politicians are of their constituents' issues, in this paper, we explore how similar politicians and their voters are in their online discourse. \gareth{I think this could benefit from some more motivation before diving into what you actually do. What is the context?}
We compare online discourse in different constituencies from both the (potential) voters and the elected politicians in the USA and UK. 
To analyze whether they talk about similar issues, we look into the variations in similarities of their online discourse through political spectrum, how contested the elections were, and impact of income. We also look into the style of their online discourse whether they talk about their political issue in same manner to convey their message effectively.

% To measure the extent of similarities in discourse after elections, In this section, we analyze similarities between content discuss on elected politician's twitter account and constituent's online discourse. We start with the similarities between topics of discussions and then move forward to analyze content similarities between their online discourse. We expect that politicians might align their online discourse \cite{colliander2017social} but also style of discourse \cite{bischof2018simple} to discuss constituents' political issues based on how contested elections are, and level of income of their constituency in national level. \gareth{I think this paragraph needs more setup text to motivate this analysis.}


% To our surprise we find that none of these has a large impact. 
% In terms of the content posted online, elected  politicians seem to be equally representative across the political spectrum, despite of the size of its victory of the level of income of the constituency.

% We then wonder whether it is more the style than the content. Could it be that elected  politicians and constituents difference on the way they talk matters more than what they actually talk about.
% We find that this is indeed the case.
% We find that there are significant differences in the way discussion happens by using LIWC categories that capture psycological factors. Hoewever, and again to our surprise, while the differences are significant they are not large.
% Indeed, we find that elected  politicians are equally representative of their constituents regardless of income and victory size.

% We finally examine the sentiment of the content they both post online, and finally we find meaningful differences.
% We find that elected  politicians and their constituents have a more similar sentiment the narrower the victory is. 
% This aligns with our intuition: the more a politician has to fight for its victory, the more likely it is that the politician will appeal to its voters by being more similar to them.
% We then examine the relationship of sentiment differences and income and again observe that the poorer the neighborhood the more representative the politician is.

% \section{Introduction}
% Elected political elected  politicians have historically relied on their national party's organization and image to attract major voter support. Nevertheless, besides national party affiliation, the constituency service is also considered a fundamental factor in electoral win \cite{jackson2005vote}. 
% With the emergence of social media platforms, politicians have started to use these platforms not just for political campaigning \cite{bossetta2023cross, brandle2022brexit}, but also
% employ these platforms to interact with constituents and tackle matters pertinent to their constituencies \cite{tromble2018thanks, baxter2016members}.

% Nevertheless, earlier research shows that elected  politicians limit discussion on issues raised by constituents with opposing views \cite{butler2016politicians} or only discuss issues that do not make them uncomfortable on social media \cite{baxter2016members}. 
% Furthermore, elected  politicians also tailor their social media communication for their impression management to their constituents \cite{jackson2020microblogging, tromble2018thanks}. These issues create a bias in elected  politicians' communication with their constituents and discussion about issues related to their constituencies. 

To study how representative elected politicians are of their constituents, we collect two large datasets:
\one Twitter timelines of elected politicians, and \two~Nextdoor posts from their respective constituents.

Nextdoor is a location-based social network with over 10 million users~\cite{nextdoor-stats}.
Nextdoor users interact within closed social networks of neighbors that have validated their home addresses, \ie a constituent posting about a local issue is in fact residing in that constituency.
We can therefore map users with their area of residence and their respective constituency.
Our Nextdoor dataset includes 21.8 Million posts from 190,706 neighborhoods (433 (98.4\%) constituencies) in the United States (USA) and 21,046 neighborhoods (595 (91.5\%) constituencies) in the United Kingdom (UK) between September 2020 and February 2023. These constituencies cover 98.6\% population in the USA and 94.6\% population in the UK.


We also collect Twitter timelines of Members of Parliament (MPs) from the UK’s House of Commons and USA Representatives (USAReps) from the USA’s House of Representatives. This includes 5.6 Million tweets from 433 USAReps’ account timelines out of 440 USAReps and 595 UK MPs’ account timelines out of 650 UK MPs.
% during almost two and a half years (September 2020 – February 2023). 

% We consider the same constituencies for our Nextdoor and Twitter data to keep our data consistent. Out of 440 USAReps, we exclude total of 7 USAReps. We exclude 5 USAReps from non-voting states that are not within the geographical boundaries of the USA. These states include American Samoa, the U.S. Virgin Islands, Guam, the Northern Mariana Islands, and Puerto Rico. We also exclude two USAReps from vacant constituencies where USAReps have deceased and no re-election has happened. Out of 650 MPs, we also exclude 55 UK MPs from our Twitter dataset who do not have a Twitter account.

Using this data, we study how representative elected politicians are of their constituency by comparing the online discourse of them both.
In particular, we address the following two Research Questions (RQs):

\begin{itemize}
    \item \textbf{RQ1:} Do elected politicians discuss similar issues of concern as their constituents? \gareth{COuld you broaden this. State that content represents issues of concern etc?}
    % (\cref{sec:income_diff})?
    \item \textbf{RQ2:} Do elected politicians follow the similar writing style as their constituents to effectively convey their message to voters?
    % ~(\cref{sec:income_inequality})?
\end{itemize}
\gareth{The above question seem a little narrow/weak. Particularly the writing style part. Could you add some motivation/context about why looking at writing style is important?}


To answer these questions, we conduct a constituency-level analysis. 
% Firstly, we observe content similarities between constituents and elected politicians across different constituencies based on income levels and level of voting majority. 
%
We find that elected politicians are frequently equally representative in terms of content and style independent of politician affiliation. The level of similarity is often low though.
Representativity is affected by how contested a constituency was in the last elections and the level of income of constituency. \gareth{Minor point. I would not write sentences in this way. You should start with the principal concern first in the sentence. E.g. here you should "Representativity is effected by...". This immediately tells the reader what the sentence is about, rather than waiting until the end to realise it.}\waleed{changed}
Elected politicians are more similar to their constituents in those constituencies that had the narrowest margins of victory. 
We find that this is true for both content and style.
This aligns well with the intuition that politicians in a contested constituency will have a strong incentive to align better with their constituents.
Although elected politicians of poorer constituencies are more representative in terms of discourse but their writing style is different from their constituents independent of how contested a constituency was in the last elections and the level of income of constituency. 
\gareth{The above is a little hard to extract a set of key messges from, particularly as concepts like "representativity" and "writing style" are a little hard to grasp at this stage.}


% We find that similarity between the contents of constituents and elected politicians is low across the USA (median cosine similarity = 0.23) and UK (median cosine similarity = 0.19) regardless of the political leaning of the constituency. We also find that constituencies with a low winning majority have greater similarity between constituents and elected politicians in the USA than in the UK. We also observe that similarity in content increases with the decreasing level of income. However, we observe that despite the low content similarity, constituents, and elected politicians discuss similar topics across the USA and UK regardless of income and voting majority level.

% We also analyze non-content-based similarities across USA and UK constituencies by observing the writing style and sentiment of content. We find that constituents and elected politicians have dissimilar styles of writing in their content but the difference is very small. Furthermore, differences in their writing style do not vary with varying income and voting majority levels. We also find that constituents and elected politicians have similar sentiments in content in low-income and low-winning majority constituencies.

This paper makes the following contributions:
\begin{itemize}
    \item Through a large-scale comparative quantitative analysis of online discourse from Nextdoor and Twitter, we show that constituents and elected politicians from the same constituency do not discuss similar content online, however, their topics of discussion are similar.
    \item We also show that their writing style in online content is dissimilar independent to political spectrum, winning majority, and income level.
    \item We also present elected politicians are relatively more similar in both content and style to their constituents in constituencies with narrowest margins of victory.
    \item We also show that elected politicians of poorer constituencies are more representative in terms of discourse.
\end{itemize}
\gareth{Expand contributions, or remove them.}\waleed{added more contributions}

